Joint processing of linguistic properties in brains and language models

Language models have been shown to be very effective in predicting brain recordings of subjects experiencing complex language stimuli. For a deeper understanding of this alignment, it is important to understand the correspondence between the detailed processing of linguistic information by the human brain versus language models. We investigate this correspondence via a direct approach, in which we eliminate information related to specific linguistic properties in the language model representations and observe how this intervention affects the alignment with fMRI brain recordings obtained while participants listened to a story. We investigate a range of linguistic properties (surface, syntactic, and semantic) and find that the elimination of each one results in a significant decrease in brain alignment. Specifically, we find that syntactic properties (i.e. Top Constituents and Tree Depth) have the largest effect on the trend of brain alignment across model layers. These findings provide clear evidence for the role of specific linguistic information in the alignment between brain and language models, and open new avenues for mapping the joint information processing in both systems. We make the code publicly available [https://github.com/subbareddy248/linguistic-properties-brain-alignment].

==> dataset.tex <==
\noindent\textbf{Brain Imaging Dataset}
The ``Narratives'' collection aggregates a variety of fMRI datasets collected while human subjects listened to naturalistic spoken stories. We analyze the ``Narratives-21\textsuperscript{st} year'' dataset~\cite{nastase2021narratives}, which is one of the largest publicly available fMRI datasets (in terms of number of samples per participant). The dataset contains data from 18 subjects who listened to the story titled ``21\textsuperscript{st} year''. The dataset for each subject contains 2226 samples (TRs-Time Repetition).
The dataset was already preprocessed and projected on the surface space (``fsaverage6'').
We use the multi-modal parcellation of the human cerebral cortex (Glasser Atlas: consists of 180 ROIs in each hemisphere) to display the brain maps~\cite{glasser2016multi}, since the Narratives dataset contains annotations that correspond to this atlas. The data covers seven language brain regions of interest (ROIs) in the human brain with the following subdivisions: (i) angular gyrus (AG: PFm, PGs, PGi, TPOJ2, and TPOJ3); (ii) anterior temporal lobe (ATL: STSda, STSva, STGa, TE1a, TE2a, TGv, and TGd); (iii) posterior temporal lobe (PTL:  A4, A5, STSdp, STSvp, PSL, STV, TPOJ1); (iv) inferior frontal gyrus (IFG: 44, 45, IFJa, IFSp); (v) middle frontal gyrus (MFG: 55b); (vi) inferior frontal gyrus orbital (IFGOrb: a47r, p47r, a9-46v), (vii) posterior cingulate cortex (PCC: 31pv, 31pd, PCV, 7m, 23, RSC); and (viii) dorsal medial prefrontal cortex (dmPFC: 9m, 10d, d32)~\cite{baker2018connectomic,milton2021parcellation,desai2022proper}.

\noindent\textbf{Extracting Word Features from BERT}
We investigate the alignment with the base pretrained BERT model, provided by Hugging Face \citep{wolf2020transformers} (12 layers, 768 dimensions). We follow previous work to extract the hidden-state representations from each layer of pretrained BERT model, given a fixed-length input length \citep{toneva2019interpreting}. To extract the stimulus features from pretrained BERT, we constrained the tokenizer to use a maximum context of previous 20 words. %with max-sequence length as 20.
Given the constrained context length, each word is successively input to the network with at most $C$ previous tokens.
For instance, given a story of $M$ words and considering the context length of 20, while the third word’s vector is computed by inputting the network with (w$_1$, w$_2$, w$_3$), the last word’s vectors w$_M$ is computed by inputting the network with (w$_{M-20}$, $\dots$, w$_M$). %\textcolor{red}{This is not entirely true since BERT takes sub-words as tokens and not words.}
The pretrained Transformer model outputs token representations at different encoder layers. We use the \#tokens $\times$ 768 dimension vector obtained from the each hidden layer to obtain word-level representations from BERT.

\noindent\textbf{Downsampling}
Since the rate of fMRI data acquisition (TR = 1.5sec) was lower than the rate at which the text stimulus was presented to the subjects, several words fall under the same TR in a single acquisition. 
Hence, we match the stimulus acquisition rate to fMRI data recording by downsampling the stimulus features using a 3-lobed Lanczos filter~\cite{lebel2021voxelwise}.
After downsampling, we average the word-embeddings within each TR to obtain the chunk-embedding corresponding to each TR. 

\noindent\textbf{TR Alignment}
To account for the slowness of the hemodynamic response, we model the hemodynamic response function using finite response filter (FIR) per voxel and for each subject separately with 8 temporal delays corresponding to 12 seconds. 

\noindent\textbf{Probing Tasks}
Probing tasks~\cite{adi2016fine,hupkes2018visualisation,jawahar2019does} help in unpacking the linguistic features possibly encoded in neural language models. In this paper, we use six popular probing tasks grouped into three categories such as surface (word length), syntactic (tree depth and top constituents), and semantic (tense, subject number, and object number) to assess the capability of BERT layers in encoding each linguistic property. 
Since other popular probing tasks such as Bigram Shift, Odd-Man-Out, and Coordination Inversion (as discussed in~\cite{conneau2018you}) have constant labels for our brain dataset, we mainly focused on six of the probing tasks mentioned above. Details of each probing task are as follows. 
\noindent\textbf{Word Length:} This surface task tests for the length of a word.
\noindent\textbf{TreeDepth:} This syntactic task tests for classification where the goal is to predict depth of the sentence's syntactic tree (with values ranging from 5 to 12). 
\noindent\textbf{TopConstituents:} This syntactic task tests for the sequence of top-level constituents in the syntactic tree. This is a 20-class classification task (e.g. ADVP\_NP\_NP\_, CC\_ADVP\_NP\_VP\_).
\noindent\textbf{Tense:} This semantic task tests for the binary classification, based on whether the main verb of the sentence is marked as being in the present (PRES class) or past (PAST class) tense. 
\noindent\textbf{Subject Number:} This semantic task tests for the binary classification focusing on the number of the subject of the main clause of a sentence. The classes are NN (singular) and NNS (plural or mass: ``colors'', ``waves'', etc). 
\noindent\textbf{Object Number:} This semantic task tests for the binary classification focusing on the object number in the main clause of a sentence. Details of these tasks are mentioned in~\cite{conneau2018you}.
\begin{table*}
\scriptsize
\centering
\caption{Probing task performance for each BERT layer before and after removal of each linguistic property using the 21$^{st}$ year stimuli.}
\label{tab:probing_results}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
 Layers & \multicolumn{2}{c|}{Word Length} & \multicolumn{2}{c|}{TreeDepth} & \multicolumn{2}{c|}{TopConstituents} & \multicolumn{2}{c|}{Tense} & \multicolumn{2}{c|}{Subject Number} & \multicolumn{2}{c|}{Object Number}  \\  
 & \multicolumn{2}{c|}{5-classes}  & \multicolumn{2}{c|}{8-classes} & \multicolumn{2}{c|}{20-classes} & \multicolumn{2}{c|}{2-classes}& \multicolumn{2}{c|}{2-classes} & \multicolumn{2}{c|}{2-classes}  \\
&  \multicolumn{2}{c|}{(Surface)} &  \multicolumn{2}{c|}{(Syntactic)} & \multicolumn{2}{c|}{(Syntactic)} & \multicolumn{2}{c|}{(Semantic)}& \multicolumn{2}{c|}{(Semantic)} & \multicolumn{2}{c|}{(Semantic)} \\\hline
&  before & after &  before & after & before & after & before & after& before & after& before & after 
\\ \hline 
1 &32.14 &03.40 & 32.41 & 13.20&42.13 & 20.71&70.53 & 53.51&86.16 & 41.80&88.39&53.94\\
2 & 30.80&14.48 &32.73 & 15.56&52.05 & 30.35&68.30 & 56.50&88.39 &54.37&85.50& 58.17 \\
3 &31.69 &17.14 &32.19 & 15.51&54.41 & 31.69&70.08 & 56.28&87.94 & 52.51&84.82&61.07\\
4 &38.83 &14.72 &30.05 & 07.73&57.01 & 22.34&69.64 & 58.07&89.41 &48.50&88.16&50.71 \\
5 &\textbf{39.73} &10.82 &32.73& 12.15&69.55& 20.55&\textbf{74.10} & 60.07&90.62 &52.07&89.28&50.16 \\
6 &39.19 &16.54 &\textbf{35.94}& 18.12&69.94& 23.58&71.43& 53.56&90.17 & 48.33&\textbf{90.17}&55.16\\
7 & 38.39& 11.94&34.01& 17.34&\textbf{80.04} &27.12&72.32& 59.30&89.28 &36.91&88.39&60.71 \\
8 &37.05 &03.52 &31.55& 09.16&79.13 &26.03&73.21 &58.28&89.73 &45.50&87.05&57.71 \\
9 &33.92 &01.70 &31.55& 07.27&72.62 &26.11&71.42 &56.26&\textbf{91.51} &54.31&88.83&56.96 \\
10 &32.58 &09.48 &31.55& 12.67&70.41 & 29.04&73.21&60.85&91.07& 53.05&88.39&55.83\\
11& 36.16&12.04 &32.62& 08.03&67.12 &28.07&71.87& 56.50&88.93 & 56.26&86.60&54.73\\
12&33.03 &10.01 &29.41 &14.13&60.05 & 24.62&73.21& 58.96&87.94 & 53.50&84.82&53.82\\
\hline
\end{tabular}
\end{table*}

\begin{figure}[t]
\centering
\includegraphics[width=0.49\linewidth]{images/task_similarity.pdf}
\includegraphics[width=0.49\linewidth]{images/balanced_task_similarity.pdf}
\caption {Task Similarity (Pearson Correlation Coefficient) constructed from the task-wise labels across six tasks.
}
\label{fig:task_correlations}
\end{figure}

\noindent\textbf{Probing Task Annotations}
To annotate the linguistic property labels for each probing task for our dataset, we use Stanford core-NLP stanza library~\cite{manning2014stanford} for sentence-level annotations. Further, for word-level annotations, we assign the same label for all the words present in a sentence except for the WordLength task.
% \textcolor{red}{For which tasks, sentence level labels are propagated to word level? Word length is word level anyway. TreeDepth ideally should be a word level property. Probably tense, subject number and object number are sentence level properties?}

\noindent\textbf{Probing Tasks Similarity}
Pearson correlation values between task labels for each pair of tasks were used to construct the similarity matrix with heatmap for the ``21st year'', as shown in Fig.~\ref{fig:task_correlations}. We observe that the following task pairs are highly correlated: (SubjNum and ObjNum), (TreeDepth and Tense), as also observed by~\citet{sileo2021analysis}.






==> limitations.tex <==
% \begin{itemize}
%     \item In this work, we explored three kinds of linguistic properties including syntax, semantic and surface types. It would be interesting to explore the role of other linguistic properties like subject-verb agreement, semantic role labeling, and also other property types like discourse based properties.
%     \item In this work, we experimented with one Transformer architecture which is the most popular (BERT). We expect the conclusions to hold good across multiple large language models, but that needs to be experimentally verified.
    
% \end{itemize}


